Calibration of the Relationship between Precipitable Water Vapor and 225 GHz Atmospheric Opacity via Optical Echelle Spectroscopy at Las Campanas Observatory

We report precipitable water vapor (PWV) measurements made at Las Campanas Observatory using optical spectra of H2O lines obtained with the Magellan echelle spectrograph, and calculated using a robust technique that is accurate to 5-10%. Calibration of the relationship between our PWV measurements and opacity values at 225 GHz was made possible by simultaneous tipping radiometer observations. Based on this calibration, we present Las Campanas Observatory winter-time precipitable water vapor statistics, measured using the tipping radiometer, during a two month campaign. The median value of 2.8 +- 0.3 mm is consistent with that measured at the nearby La Silla Observatory during the VLT site survey. We conclude that, in the Southern hemisphere winter months, we can expect good conditions for infrared observing (<~1.5 mm) approximately 10% of the time at Las Campanas Observatory.

==> tab1.tex <==
\begin{deluxetable}{rrrcccl}
\tablenum{1}
\tablewidth{0pt}
\tablecaption{Log of Observations}
\tablehead{\colhead{Obs. \#} & \colhead{HR \#} & \colhead{UT Date} & \colhead{UT Start} & \colhead{Airmass} & \colhead{Exp. (sec)} &
\colhead{Observer\tablenotemark{*} } }
\startdata
1   & 5987  & 21/Jul/2005 &  22:49  &  1.116 & 24 & ALM   \cr
2   & 5987  & 22/Jul/2005 &  22:46  &  1.115 & 32 & ALM   \cr
3   &  806  & 24/Jul/2005 &  11:01  &  1.292 & 30 & ALM   \cr
4   & 5987  & 25/Jul/2005 &  01:37  &  1.033 & \hskip6pt 5 & AD    \cr
5   & 845   & 30/Jul/2005 &  10:42  &  1.002 & 15 & IT    \cr
6   & 5517  & 30/Jul/2005 &  22:44  &  1.002 & 15 & IT    \cr
7   & 5517  &  1/Aug/2005 &  22:48  &  1.001 & 15 & IT    \cr
8   & 5517  &  2/Aug/2005 &  23:08  &  1.005 & 15 & IT    \cr
9   & 6930  & 20/Aug/2005 &  01:52  &  1.043 & 15 & GWP   \cr
10  & 5987  & 20/Aug/2005 &  23:10  &  1.011 & 32 & GWP   \cr
11  & 5987  & 23/Aug/2005 &  23:08  &  1.014 & 62 & GWP   \cr
12  & 5987  & 24/Aug/2005 &  22:52  &  1.011 & 30 & GWP   \cr
13  & 6930  & 15/Sep/2005 &  01:00  &  1.098 & 10 & KL    \cr
14  & 8998  & 21/Nov/2005 &  23:45  &  1.030 & 49 & AMcW  \cr
15  & 3034  & 22/Nov/2005 &  08:21  &  1.002 & \hskip6pt 3 & NM    \cr

\enddata
\tablenotetext{*}{Observer key: AD (Andrea Dupree), IT (Ian Thompson), GWP (George Preston),
KL (Kulkarni \& Lauroesch), AMcW (Andrew McWilliam), NM (Nidia Morel), 
ALM (Adams \& Lopez Moralez)}
\label{tab-log}
\end{deluxetable}


==> tab2.tex <==
\begin{deluxetable}{cccllcc}
\tablenum{2}
\tablewidth{0pt}
\tablecaption{Parameters of Temperature Insensitive H$_2$O Lines\tablenotemark{*}}
%\tablehead{\colhead{$\sigma_{\rm vac}$ (cm$^{-1}$)}  & \colhead{$\lambda_{\rm air}$ (\AA )}
%        &  \colhead{ EP (cm$^{-1}$)}                 & \colhead{gf} 
%       &  \colhead{S$_{270}$ (cm$^{-2}$)}  & EW$_{dry}$ (m\AA )  & EW$_{wet}$ (m\AA ) \cr
\tablehead{\colhead{$\sigma_{\rm vac}$}  & \colhead{$\lambda_{\rm air}$}
        &  \colhead{EP}                 & \colhead{gf} 
       &  \colhead{S$_{270}$}  & \colhead{EW$_{dry}$}   & \colhead{EW$_{wet}$} \cr

\colhead{(cm$^{-1}$)}  & \colhead{(\AA )}
        &  \colhead{(cm$^{-1}$)}                 & 
       &  \colhead{(cm$^{-2}$)}  & \colhead{(m\AA )}  & \colhead{(m\AA )} 
}
\startdata
13717.1744  &  7288.10  &  275.50  & 5.323$\times$10$^{-9}$   & 0.2387 &  6 &  88 \cr
13718.5755  &  7287.36  &  300.36  & 1.251$\times$10$^{-8}$   & 0.4912 & \llap{2}1 & \llap{1}34 \cr
13823.1810  &  7232.21  &  300.36  & 5.602$\times$10$^{-9}$   & 0.2200 &  9 &  75 \cr
13894.6353  &  7195.02  &  285.42  & 6.159$\times$10$^{-9}$   & 0.2619 & \llap{1}2 &  84 \cr
14397.3641  &  6943.79  &  224.84  & 3.059$\times$10$^{-9}$   & 0.1795\rlap{\tablenotemark{**}}  & 5\rlap{:} &  52 \cr
16788.1104  &  5954.94  &  300.36  & 8.942$\times$10$^{-10}$  & 0.03511 & ... &  \hskip6pt 6 \cr
\enddata
\tablenotetext{*}{S and gf values calculated from Coheur et al. (2002) A values.}
\tablenotetext{**}{Compares well with Brault et al. (1975) S value of 0.180.}
\label{tab-params}
\end{deluxetable}


==> tab3.tex <==
\begin{deluxetable}{r|cc|cc|cc|cc|cc|cc|cc}
\rotate
\tablenum{3}
\tablecolumns{15}
\tablewidth{0pt}
\tablecaption{Line Fluxes\tablenotemark{*} and PWV Values}
\tablehead{
\colhead{Obs.}  &
\multicolumn{2}{c}{7288.10\AA}   &        \multicolumn{2}{c}{7287.36\AA}       &  
          \multicolumn{2}{c}{7232.21\AA}     &  \multicolumn{2}{c}{7195.02\AA}      &     \multicolumn{2}{c}{6943.78\AA}      &
          \multicolumn{2}{c}{5954.94\AA\tablenotemark{\ddag}}     &  \colhead{$\overline{\rm PWV}$\tablenotemark{\dag} (mm)} & \colhead{$\sigma$}  \cr
     &     \colhead{$-$ln F} &  \colhead{PWV} &  \colhead{$-$ln F} &  \colhead{PWV} &  \colhead{$-$ln F} &  \colhead{PWV} &
           \colhead{$-$ln F} &  \colhead{PWV} &  \colhead{$-$ln F} &  \colhead{PWV} &  \colhead{$-$ln F} &  \colhead{PWV} & & }
\startdata
 1   &    ...   &  ...   &    ...   &  ...  &   0.036\rlap{:} & 1.47  &  0.047\rlap{:} & 1.61  &    0.041   & 2.05  &      ...    &   ... &     1.71  &  0.30  \cr
 2   &    ...   &  ...   &    ...   &  ...  &   0.032\rlap{:} & 1.31  &  0.031\rlap{:} & 1.06  &    0.028   & 1.40  &      ...    &   ... &     1.26  &  0.17  \cr
 3   &    ...   &  ...   &    ...   &  ...  &    ...   &  ...  &  0.039\rlap{:} & 1.15  &    0.019\rlap{:}  & 0.82  &      ...    &   ... &     0.99  &  0.24  \cr
 4   &   0.013\rlap{:} & 0.53   &   0.044  & 0.87  &   0.023\rlap{:} & 1.01  &  0.027\rlap{7} & 1.00  &    0.027   & 1.19  &      ...    &   ... &     0.97  &  0.30  \cr
     &          &        &          &       &          &       &         &       &    0.017\rlap{:}  &       &             &       &           &        \cr
 5   &   0.122  & 5.10   &   0.216  & 4.39  &   0.116  & 4.92  &  0.126  & 4.80  &    0.095   & 4.92  &     0.022\rlap{:}  &  5.26 &     4.85  &  0.36  \cr
     &          &        &          &       &   0.101  &       &         &       &    0.082   &       &     0.015   &       &           &        \cr
 6   &   0.110  & 4.60   &   0.196  & 3.98  &   0.098  & 4.12  &  0.127  & 4.84  &    0.079   & 4.42  &     0.011\rlap{:}  &  3.13 &     4.36  &  0.32  \cr
     &          &        &          &       &   0.087  &       &         &       &    0.080   &       &     0.011   &       &           &        \cr
 7   &   0.093  & 3.89   &   0.184  & 3.74  &   0.085  & 3.79  &  0.100  & 3.81  &    0.060   & 3.68  &     0.013   &  3.70 &     3.77  &  0.21  \cr
     &          &        &          &       &   0.082  &       &         &       &    0.072   &       &             &       &           &        \cr
 8   &   0.184  & 7.67   &   0.293  & 5.94  &   0.166  & 7.17  &  0.190  & 7.22  &    0.127   & 6.90  &     0.295\rlap{:}  &  6.84 &     7.00  &  0.57  \cr
     &          &        &          &       &   0.151  &       &         &       &    0.122   &       &     0.188   &       &           &        \cr
 9   &   0.064  & 2.57   &   0.123  & 2.40  &   0.063  & 2.94  &  0.063  & 2.31  &    0.048   & 2.30  &     0.008\rlap{::} &  2.18 &     2.54  &  0.35  \cr
     &          &        &          &       &   0.072  &       &         &       &    0.038   &       &             &       &           &        \cr
10   &   0.063  & 2.61   &   0.121  & 2.44  &   0.065  & 2.95  &  0.067  & 2.53  &    0.049   & 2.45  &      ...    &   ... &     2.63  &  0.27  \cr
     &          &        &          &       &   0.066  &       &         &       &    0.040   &       &             &       &           &        \cr
11   &   0.101  & 4.17   &   0.190  & 3.81  &   0.095  & 4.35  &  0.101  & 3.80  &    0.073   & 3.87  &      ...    &   ... &     4.03  &  0.27  \cr
     &          &        &          &       &   0.099  &       &         &       &    0.068   &       &             &       &           &        \cr
12   &   0.085  & 3.52   &   0.158  & 3.18  &   0.075  & 3.64  &  0.083  & 3.14  &    0.061   & 3.20  &      ...    &   ... &     3.36  &  0.30  \cr
     &          &        &          &       &   0.087  &       &         &       &    0.055   &       &             &       &           &        \cr
13   &   0.040  & 1.53   &   0.076  & 1.30  &   0.036  & 1.49  &  0.040  & 1.39  &    0.033   & 1.60  &      ...    &   ... &     1.49  &  0.12  \cr
     &          &        &          &       &   0.036  &       &         &       &    0.030   &       &             &       &           &        \cr
14   &    ...   &  ...   &   0.122\rlap{:} & 2.44  &   0.034\rlap{:} & 1.63  &   ...   &  ...  &    0.037   & 2.40  &      ...    &   ... &     2.10  &  0.54  \cr
     &          &        &          &       &   0.038  &       &         &       &    0.052\rlap{:}  &       &             &       &           &        \cr
15   &   0.050  & 2.03   &   0.094  & 1.78  &   0.052  & 2.19  &  0.058  & 2.15  &    0.036   & 2.00  &      ...    &   ... &     2.05  &  0.17  \cr
     &          &        &          &       &   0.047  &       &         &       &    0.036   &       &             &       &           &        \cr
\enddata
\label{tab-pwv}
\tablenotetext{*}{\ Flux measurements for lines appearing in a second order are indicated below the first entry}
\tablenotetext{\dag}{\ Lines appearing in two orders were counted twice for the calculation of the average PWV}
\tablenotetext{\ddag}{\ The 5954.94\AA\ line was not used for the average PWV}
\end{deluxetable}


==> tab4.tex <==
\begin{deluxetable}{cccllr}
\tablenum{4}
\tablewidth{0pt}
\tablecaption{Parameters for Strong H$_2$O Lines}
%\tablehead{\colhead{$\sigma_{\rm vac}$ (cm$^{-1}$)}  & \colhead{$\lambda_{\rm air}$ (\AA )}
%        &  \colhead{ EP (cm$^{-1}$)}                 & \colhead{gf} 
%       &  \colhead{S$_{270}$ (cm$^{-2}$)}  & EW$_{dry}$ (m\AA )  & EW$_{wet}$ (m\AA ) \cr
\tablehead{\colhead{$\sigma_{\rm vac}$}  & \colhead{$\lambda_{\rm air}$}
        &  \colhead{EP}                 & \colhead{gf} 
       &  \colhead{S$_{270}$}  & \colhead{EW$_{wet}$} \cr

\colhead{(cm$^{-1}$)}  & \colhead{(\AA )}
        &  \colhead{(cm$^{-1}$)}                 & 
       &  \colhead{(cm$^{-2}$)}  & \colhead{(m\AA )} 
}
\startdata
10704.4205  &  9339.33  & 300.36   & 2.730$\times$10$^{-7}$   &  10.7240\tablenotemark{2}  &  1047. \cr
11002.2178  &  9086.55  & 285.22   & 1.245$\times$10$^{-8}$   &   0.5303\tablenotemark{2}  &   186. \cr
11124.6353  &  8986.56  & 300.36   & 3.017$\times$10$^{-8}$   &   1.1852\tablenotemark{2}  &   343. \cr
12254.5139  &  8157.99  & 300.36   & 1.676$\times$10$^{-8}$   &   0.6584\tablenotemark{1}  &   208. \cr
11096.9124  &  9009.01  & 285.22   & 4.443$\times$10$^{-9}$   &   0.1892\tablenotemark{2}  &   111. \cr
12238.3078  &  8168.79  & 222.05   & 7.226$\times$10$^{-9}$   &   0.4309\tablenotemark{1}  &   180. \cr
12062.4127  &  8287.91  & 224.84   & 1.770$\times$10$^{-8}$   &   1.0397\tablenotemark{1}  &   313. \cr
12037.5135  &  8305.05  & 325.35   & 2.243$\times$10$^{-8}$   &   0.7714\tablenotemark{1}  &   241. \cr
\enddata
\tablenotetext{1}{S and gf values calculated from Coheur et al. (2002) A values.}
\tablenotetext{2}{S and gf values calculated from Brown et al. (2002) A values.}
\label{tab-strong}
\end{deluxetable}


==> tab5.tex <==
\begin{deluxetable}{lrrrl}
\tablenum{5}
\tablewidth{0pt}
\tablecaption{Comparison of calibration at LCO to that at other sites}
\tablehead{\colhead{Site} & \colhead{Altitude (km)} & \colhead{$\tau_{dry-air}$} & \colhead{B} & \colhead{Reference}}
\startdata
LCO Alcaino  & 2410  & 0.015$\pm$0.013 &  0.076$\pm$0.005  &  this work \cr
S. Pole  & 2835  & 0.026$\pm$0.001\tablenotemark{*} &  0.083$\pm$0.002\tablenotemark{*}  &  \citet{cha04} \cr
Mauna Kea & 4100 & 0.016 & 0.05 & \citet{dav97} \cr
Llanno de Chanjantor & 5104 & 0.0068 & 0.0407 & \citet{del99} \cr
\enddata
\tablenotetext{*}{uncertainties from \citet{cb95}}
\label{tab-cal}
\end{deluxetable}

